Computational Limitations in Robust Classification and Win-Win Results

We continue the study of statistical/computational tradeoffs in learning robust classifiers, following the recent work of Bubeck, Lee, Price and Razenshteyn who showed examples of classification tasks where (a) an efficient robust classifier exists, in the small-perturbation regime; (b) a non-robust classifier can be learned efficiently; but (c) it is computationally hard to learn a robust classifier, assuming the hardness of factoring large numbers. The question of whether a robust classifier for their task exists in the large perturbation regime seems related to important open questions in computational number theory. In this work, we extend their work in three directions. First, we demonstrate classification tasks where computationally efficient robust classification is impossible, even when computationally unbounded robust classifiers exist. For this, we rely on the existence of average-case hard functions. Second, we show hard-to-robustly-learn classification tasks in the large-perturbation regime. Namely, we show that even though an efficient classifier that is robust to large perturbations exists, it is computationally hard to learn any non-trivial robust classifier. Our first construction relies on the existence of one-way functions, and the second on the hardness of the learning parity with noise problem. In the latter setting, not only does a non-robust classifier exist, but also an efficient algorithm that generates fresh new labeled samples given access to polynomially many training examples (termed as generation by Kearns et. al. (1994)). Third, we show that any such counterexample implies the existence of cryptographic primitives such as one-way functions. This leads us to a win-win scenario: either we can learn an efficient robust classifier, or we can construct new instances of cryptographic primitives.

==> ecc-prf.tex <==
% !TeX root = ms.tex
\section{Using Pseudorandom Functions and Error Correcting Codes}

In this section, we formally describe the hard-to-robustly learn task based on one-way functions. There are two main ingredients that we use to construct the learning task: Error Correcting Codes (ECCs) and Pseudorandom Functions (PRFs).

An uniquely decodable binary error correcting code allows encoding messages to redundant codewords such that from any codeword perturbed to some degree, we can recover the encoded message.

\begin{definition}[Uniquely Decodable Error Correcting Code]
An uniquely decodable binary error correcting code, $ C : \zo^n \rightarrow \zo^m $ consists of two efficient algorithms $ \encode, \decode $. The code tolerates error fraction $ e $ if for all messages $ x\in \zo^n $,  	$$ \decode(\tilde y) =  x \text{ for all $ \tilde y \in B(\encode(x), em)$}$$
where $ B(\encode(x), em) $ denotes the Hamming ball of radius $ em $.
\end{definition}

We know very good error correcting codes.
\begin{theorem}[\cite{GI01}] For any constant $ \gamma > 0 $, there exists a binary error correcting code $ C: \zo^{n} \rightarrow \zo^{m} $ where $ m=O(n/\gamma^3) $ with a decoding radius of $ (\frac14 - \gamma) m$ with polynomial time encoding and decoding.
\end{theorem}
We will use this coding scheme with $ \gamma = 1/8 $ giving us an error correcting code $ C: \zo^n \rightarrow \zo^m $ where $ m = \theta(n) $ and tolerates $ m/8 $ errors for unique decoding.

A \textdef{pseudorandom function} is a keyed function $ F_k : \zo^{n-1} \rightarrow \zo$ where the secret key is picked uniformly random such that, for every efficient adversary, the output of the function is indistinguishable from the output of a random function.  A more formal definition is given below. It is known that pseudorandom functions can be constructed from one-way functions.
\begin{definition}[\cite{GGM86}]
A family of polynomial-time computable functions $\cF= \set{\cF_n}$ where  $\cF_n = \set{F_{k} : \zo^n \rightarrow \zo } $ where $ k \in \zo^n $ and $ n \in \NN $ is \textdef{pseudorandom} if every polynomial time computable adversary $ \sfA $ cannot distinguish between $ \cF $ and uniformly random function. That is,
\[ \abs{\prob[k\gets \zo^n]{\sfA^{F_k}(1^n) = 1 } - \prob[U_n \gets \cU_n]{\sfA^{U_n}(1^n) = 1 }} < \negl(n)\]
where $ \cU_n $ is the uniform distribution over all functions from $ \zo^n $ to $ \zo $.
\end{definition}
\begin{theorem}[\cite{GGM86}] Pseudorandom functions exist if one-way functions exist.
\end{theorem}

Next, we informally describe the learning task.
Consider the following learning task: The two distributions $ D_0, D_1 $ are parameterized by the PRF key $ k $ and defined as follows:
\[ D_0 = (0, \encode(x, F_k(x))) \text{ and, } D_1 = (1, \encode(x, 1- {F_k(x)})) \ .\]
So, the two distributions are tuples where the first half is which distribution the sample was taken from and the second an error correcting code applied to the tuple $ (x, F_k(x) + b) $, that is, either the PRF evaluation at the location $ x $ or its complement.
Note that without the first bit, classifying the original distributions is computationally infeasible. The pseudorandom function looks random at every new location. Including the bit in the sample itself makes the unperturbed classification task easy. The error correcting code ensures that we have a robust classifier.

\begin{theorem}
\label{thm:prfs}
Let $ \set{F_k} $ for $ F_k : \zo^{n-1} \rightarrow \zo $  be a pseudorandom function family and $ C : \zo^n \rightarrow \zo^m $ where $ m = \theta(n) $ be an efficiently decodable error correcting code  with decoding algorithm $ \sf{Decode} $ that tolerates $ m/8 $ errors.

Consider the following learning task. For a random pseudorandom function key $ k $, define:
$$ D^{(k)}_0 = \set{(0, C(x, F_k(x))) : x\gets \zo^{n-1}} \text{ and, }D^{(k)}_1 = \set{(1, C(x, 1-F_k(x))) : x\gets \zo^{n-1}} $$
supported on $ \zo^m $. The learning task has the following properties.
\begin{enumerate}
\item (Easy to Learn) A classifier to distinguish $ D_0 $ from $ D_1 $ can be learned from the samples efficiently.
\item (Robust Classifier Exists) There exists a robust classifier $ \sfR $ such that, \[ \prob[y\gets D_b]{B(y, m/8) \in \sfR^{-1}(b)} \geq 0.99 \]
where $ m/8 $ is the decoding radius and $ B(y, d)  = \{y' : \|y-y'\|_{\sf{Ham}} \leq d \}$.
\item (A Robust Classifier is hard-to-learn) There exists a perturbation algorithm such that no efficiently learned classifier can classify perturbed adversarial examples better than chance.
\end{enumerate}
\end{theorem}
\begin{proof}
To prove Part (1) consider the classifier that outputs the first bit. It works correctly on instances from the distributions.
To prove Part (2), we rely on the decoding algorithm. After $ d = m/8 $ edits to the sample, we can recover the underlying message by ignoring the first bit of the tuple and decoding the rest to get the underlying message of the form $ (x, c) $ and then use the PRF to classify. More formally, consider the following robust classifer:

\noindent
\begin{minipage}{0.8\textwidth}
	\medskip
	\underline{\sf{Robust Classifer} $ \sfR_{k}(\tilde{{y}}) $ where $ \tilde y \in \zo^{m+1} $}:
	\begin{enumerate}[noitemsep,nolistsep]
		\item Let $ (x, c) = \mathsf{Decode}(\tilde{y}_{2:m+1}) $ where $ \tilde{y}_{2:m+1} $ are all of $ \tilde y $ but the first bit.
		\item Output $ 0 $ if $ c = F_k(x) $ else output 1.
	\end{enumerate}
	\medskip
\end{minipage}

Observe that error correcting code ensures that from every perturbed sample, we efficiently recover the encoded message. And then because the message is of the form $ (x, F_k(x) + b) $ for class $ b $, this allows for correct classification.

To show Part (3), we rely on the unlearnability of the PRF. Consider a perturbing adversary that replaces the first bit of the sample by 0. Classification is now equivalent to predicting $ F_k(x) $ given $ x $. %Given any classifier, the predictor for $ F_k(x) $ is to encode $ (x,0) $ and feed it to the classifer and use this label to predict $ F_k(x) $.
Because predicting $ F_k(x) $ is computationally infeasible to learn, so is a robust classifier.
\end{proof}

Note that, compared to the previous counter-examples, this example does not rely on public key assumptions. The reason for that is that the samples here are ``evasive''. In that there is no way to generate fresh samples from the two distributions. So, we cannot translate this to a public key encryption scheme because to encrypt, we need a samples from the distributions $ D_0, D_1$ along with the perturbing adversary and we do not have access to these samples.

The hardness of this task comes from the hardness of learning the PRF and not from the perturbations. This is different from the schemes based on LPN and LWE.

